HEIDL: Learning Linguistic Expressions with Deep Learning and Human-in-the-Loop

While the role of humans is increasingly recognized in machine learning community, representation of and interaction with models in current human-in-the-loop machine learning (HITL-ML) approaches are too low-level and far-removed from human's conceptual models. We demonstrate HEIDL, a prototype HITL-ML system that exposes the machine-learned model through high-level, explainable linguistic expressions formed of predicates representing semantic structure of text. In HEIDL, human's role is elevated from simply evaluating model predictions to interpreting and even updating the model logic directly by enabling interaction with rule predicates themselves. Raising the currency of interaction to such semantic levels calls for new interaction paradigms between humans and machines that result in improved productivity for text analytics model development process. Moreover, by involving humans in the process, the human-machine co-created models generalize better to unseen data as domain experts are able to instill their expertise by extrapolating from what has been learned by automated algorithms from few labelled data.

==> interviews.tex <==
\section{Formative Study}
 To further inform the user experience of our tool we conducted informal studies with expert text analytics researchers (2) and developers (4). 
 
 Subjects stated that understanding the domain of interest, concepts and relationships is crucial in  sketching semantic patterns.  Recall is identified to be by far the most difficult part of the whole process, compared to precision. As for experiences with machine learning so far, experts commented that they typically overfit over training data and do very poorly on another dataset. Even worse, whatever experts learn in one domain hardly ever translates to another domain, and as such delivering solutions in another domain is work almost starting from scratch. Subjects expressed desire to build trust with machine-learned models, to have more playground where they could examine parts of rules, add and remove predicates, examine changes in output and quality. As for  rules subjects preferred shorter generalizable rules over   specific rules that tend to overfit. Another important takeaway  was that experts really need more help, one expert said that ``tooling in this space is really undervalued", and added that ``HITL should be groomed in", suggesting that novel ways to engage experts with machine-learning has a lot of potential, especially if machine learning output makes sense semantically, can be examined, and used as a starting point to play with the model. 


